Preference Learning Algorithms Do Not Learn Preference Rankings

Preference learning algorithms (e.g., RLHF and DPO) are frequently used to steer LLMs to produce generations that are more preferred by humans, but our understanding of their inner workings is still limited. In this work, we study the conventional wisdom that preference learning trains models to assign higher likelihoods to more preferred outputs than less preferred outputs, measured via ranking accuracy. Surprisingly, we find that most state-of-the-art preference-tuned models achieve a ranking accuracy of less than 60% on common preference datasets. We furthermore derive the idealized ranking accuracy that a preference-tuned LLM would achieve if it optimized the DPO or RLHF objective perfectly. We demonstrate that existing models exhibit a significant alignment gap -- i.e., a gap between the observed and idealized ranking accuracies. We attribute this discrepancy to the DPO objective, which is empirically and theoretically ill-suited to fix even mild ranking errors in the reference model, and derive a simple and efficient formula for quantifying the difficulty of learning a given preference datapoint. Finally, we demonstrate that ranking accuracy strongly correlates with the empirically popular win rate metric when the model is close to the reference model used in the objective, shedding further light on the differences between on-policy (e.g., RLHF) and off-policy (e.g., DPO) preference learning algorithms.

==> sections_theoretical_foundations/discussion.tex <==
Our work highlights the significant but nuanced relationship between preference learning and ranking accuracy. 
We have demonstrated both theoretically and empirically that RLHF and DPO struggle to teach the model to correctly rank preferred and dispreferred outputs, even in the training dataset. Although the learning objective promotes high ranking accuracy in theory (\cref{prop:sanity_check}), we observed a prominent \emph{alignment gap} resulting from the poor conditioning of reference models. We then drew connections between the off-policy nature of ranking accuracy and the on-policy evaluations of win rate, identifying specific scenarios in which on-policy behavior can or cannot be reliably predicted by off-policy behavior. App.~\ref{sec:app_discussion} describes the limitations of our work and the important implications for AI safety.
%More practically speaking, our work also suggests a simple method for identifying training examples that a model may struggle to learn, and motivates both the use of stronger $\pi_\text{Ref}$ models and iterative or on-policy variants of DPO~\citep{tang2024generalized,yuan2024selfrewarding,kim2024sdpo,tran2023iterative}. % \ac{cite!}. 

% relationship between RA and WR motivate the use of "iterative" RLHF/DPO algorithms, and other on-policy/online training algs



==> sections_theoretical_foundations/idealized.tex <==
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/rank_accs_ref_models.pdf}
        \caption{Ranking accuracies of various reference models, including \textsc{GPT2} \citep{radford2019language}, \textsc{Pythia 1.4B} and \textsc{2.8B} \citep{biderman2023pythia}, \textsc{Llama 2 7B} \citep{touvron2023llama}, \textsc{Vicuna 1.5 7B} \citep{zheng2023judging}, \textsc{OLMo 7B} \citep{OLMo}, \textsc{Tulu2 7B} \citep{ivison2023camels}, \textsc{Zephyr 7B SFT} \citep{alignment_handbook2023}, \textsc{Mistral v0.1 7B} \citep{jiang2023mistral}, and \textsc{Gemma 7B} \citep{gemmateam2024gemma}.}
        \label{fig:ranking-acc-ref-models}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/rank_accs_pref_models.pdf}
        \caption{Ranking accuracies of various preference-tuned models, including \textsc{Llama 2 7B Chat} \citep{touvron2023llama}, \textsc{Tulu2 7B DPO} \citep{ivison2023camels}, \textsc{Zephyr 7B DPO} \citep{alignment_handbook2023}, and \textsc{Gemma 7B IT} \citep{gemmateam2024gemma}}
        \label{fig:ranking-acc-pref-models}
        \vspace{30pt}
    \end{subfigure}
    \caption{\textbf{Both reference and preference-tuned models exhibit low ranking accuracy on most preference datasets.} Each point represents the length-normalized or non-length-normalized ranking accuracy of individual (\ref{fig:ranking-acc-ref-models}) reference models (pre-trained or fine-tuned), or (\ref{fig:ranking-acc-pref-models}) preference-tuned models (trained with DPO or RLHF). We sub-sample 1K examples from each dataset and use the test split when available. We describe datasets in \ref{sec:datasets} and list all numbers in Tables \ref{tab:ra-full-pt1}, \ref{tab:ra-full-pt2}, and \ref{tab:ra-full-pt3}.}
    \label{fig:ranking-accs}
\end{figure*}

Prop. \ref{prop:sanity_check} showed that training a low DPO loss with a perfect reference model yields a model with perfect ranking accuracy.
%, but only if the reference model already achieves perfect ranking accuracy. 
%However, Fig.~\ref{fig:ranking-acc-ref-models} shows that real-world reference models exhibit low ranking accuracies, which prompts us to
%\Cref{prop:sanity_check} identifies two conditions for high ranking accuracy: (1) a reference model $\refmodel$ with the correct ranking on completions, and (2) a low value of $\dpoloss$.
%As such, in this section, we 
%study %the gap between empirically observed ranking accuracies and the ranking accuracies predicted by the theory in 
%more realistic, imperfect reference models.%, and understanding the contributors to this gap.
However, we observe that reference models rarely achieve high ranking accuracy on common preference datasets (Fig.~\ref{fig:ranking-acc-ref-models}).\footnote{We cannot be sure if these datasets were in-distribution for these models, because the training details are not public.}
This finding is especially concerning because the DPO objective and RLHF reward were formulated to ensure the model learns the preference dataset without straying too far from the reference model.
We formalize this limitation of the alignment objectives by studying what the optimal policies would be when perfectly optimizing DPO or RLHF with access to perfect data.
\begin{theorem}[Simulating Perfect RLHF\footnote{We note that this result can also be straightforwardly derived from prior works~\citep{peters2007reinforcement,korbak2022rl,go2023aligning}.}]\label{thm:upper_bound}
    Fix a reference model $\refmodel$ and an aggregated preference datapoint $(x, y_w, y_l)\sim\gD$. Assume the dataset includes the ground-truth human preferences: that is, $\alpha(x, y_w, y_l)=\mathbb{P}(y_w\succ y_l)$, and that these preferences obey the Bradley-Terry model (\Cref{assume:bt}). Let $\pi^*$ be the model resulting from perfectly optimizing the DPO or RLHF objective on $(x, y_w, y_l)$ as described in~\Cref{subsec:prelims_preferences}. Then, $\pi^*$ satisfies
    \begin{equation}
        \frac{\pi^*(y_w\mid x)}{\pi^*(y_l\mid x)} = \frac{\refmodel({y_w\mid x})}{\refmodel(y_l\mid x)} \left(\frac{\alpha(x, y_w, y_l)}{1-\alpha(x, y_w, y_l)}\right)^{1/\beta}
    \end{equation}
    where $\alpha(x, y_w, y_l)$ is the proportion of raters who preferred $y_w$ over $y_l$ and $\beta$ is a hyperparameter in the DPO and RLHF objectives.
\end{theorem}
We prove this result in App. \ref{sec:proof-upper-bound}.
Our result allows us to compute the idealized ranking accuracy, denoted $\idealrankacc$, when training on a given preference dataset $\gD$ with a reference model $\refmodel$ (\Cref{cor:idealized_rank_acc}).
We report the idealized ranking accuracy of various open-access models in Table \ref{tab:ranking_accs} and further details are given in App. \ref{app:comp-idealized-ra}.\footnote{Note that when $\alpha(x, y_w, y_l) = 1$, we replace it with $1-\epsilon$ to compute the formula. We also test a range of $\beta$ values, since the choice of $\beta$ was not released for these models. See App. \ref{app:comp-idealized-ra}.} 
Even under ideal conditions (\emph{i.e.} perfectly optimizing the objective on ground-truth preference data), the idealized ranking accuracy is still sometimes below $100\%$. 
This distance varies with the choice of $\beta$, which indicates that the limits of DPO/RLHF depend largely upon how strong the reliance on $\pi_\text{Ref}$ is. 
Furthermore, we find that many state-of-the-art models do not achieve a ranking accuracy anywhere close to the idealized ranking accuracy, exhibiting alignment gaps ranging from 19 to 59 percentage points (measured to the median idealized $\rankacc$ or $\tilde\rankacc$).
%The results are shown in Table \ref{tab:ranking_accs} and further details are given in App. \ref{app:comp-idealized-ra}.

%First, we demonstrate that reference models rarely rank completions correctly, even if they are trained on the preferred completions (see~\Cref{subsec:prelims_preferences}).
%Then, we derive what the optimal policies are after training on infinite preference data (i.e., when $\alpha(x, y_1, y_2) = \Pr[y_1\succ y_2]$), which allows us to describe the ranking accuracy of the model after preference learning under ideal conditions.
%This idealized ranking accuracy is cheap and straightforward to compute, requiring access only to the reference model $\refmodel$ and the preference dataset $\gD$.
%Measurements on Alpaca-Eval~\citep{li2023alpacaeval} show that the accuracy of several common models under idealized conditions is less than $1$, and the true ranking accuracy of the models is less than $50\%$.
%Our findings altogether indicate an impossibility to fully align existing models to a training dataset.





\iffalse
\subsection{Existing Reference Models Rarely Have Correct Rankings}\label{sec:ref_model_ranking}

%With the exception of the Synthetic Instruct GPT-J Pairwise dataset, 
Fig. \ref{fig:ranking-acc-ref-models} indicates that reference models rarely achieve high ranking accuracy on common preference datasets (except Synthetic Instruct GPT-J Pairwise), even though many were likely trained on the preferred completions (see Sef. \ref{subsec:prelims_preferences}). 
Many of the models do not have documented training data so we do not know which preference datasets, if any, are in-distribution.
%However, since many of the creators of these models have not released the full set of datasets that the models were trained on, we cannot be sure whether these preference datasets are in-distribution. 
We also fine-tune several pretrained LLMs on the preferred completions (see App. \ref{app:ra-open-source-custom-eval}) and observe that ranking accuracy does not increase significantly.\footnote{It is not surprising that fine-tuning on the preferred completions does not boost ranking accuracy, since the model does not receive any knowledge of the relative qualities of the preferred and rejected completions.}
Based on our findings, we turn to the case of imperfect reference models.
%This finding leads us to study the case where the reference model has incorrect rankings. 

\subsection{Idealized Ranking Accuracy}
%\sm{Difference between this and sanity check proposition}
We showed above that empirically, reference models exhibit poor accuracy when ranking the plausible completions.
However, the RLHF reward and DPO objective were formulated to ensure that the model learns the preference dataset but does not move too far from the  reference model $\refmodel$, so there may be a limit on the possible accuracy of the preference-tuned model.
Here, we formalize this intuition by studying what the optimal policies would be when perfectly optimizing DPO or RLHF with access to perfect data (i.e., true proportions of human preferences).\footnote{This result differs from \Cref{prop:sanity_check} in that it accounts for a potentially imperfect reference model.}
\begin{theorem}[Simulating Perfect RLHF\footnote{We note that this result can also be straightforwardly derived from prior works~\citep{peters2007reinforcement,korbak2022rl,go2023aligning}.}]\label{thm:upper_bound}
    Fix a reference model $\refmodel$ and an aggregated preference datapoint $(x, y_w, y_l)\sim\gD$. Assume the dataset includes the ground-truth human preferences: that is, $\alpha(x, y_w, y_l)=\mathbb{P}(y_w\succ y_l)$, and that these preferences obey the Bradley-Terry model (\Cref{assume:bt}). Let $\pi^*$ be the model resulting from perfectly optimizing the DPO or RLHF objective on $(x, y_w, y_l)$ as described in~\Cref{subsec:prelims_preferences}. Then, $\pi^*$ satisfies
    \begin{equation}
        \frac{\pi^*(y_w\mid x)}{\pi^*(y_l\mid x)} = \frac{\refmodel({y_w\mid x})}{\refmodel(y_l\mid x)} \left(\frac{\alpha(x, y_w, y_l)}{1-\alpha(x, y_w, y_l)}\right)^{1/\beta}
    \end{equation}
    where $\alpha(x, y_w, y_l)$ is the proportion of raters who preferred $y_w$ over $y_l$ and $\beta$ is a hyperparameter in the DPO and RLHF objectives.%\footnote{Proof in \ref{sec:proof-upper-bound}}
    %and $\epsilon$ is a very small constant.
%    \sm{Rephrase this to concentrate on $\alpha$}
    %\sm{We should stabilize the denominator I think}
\end{theorem}

\begin{remark}
    We prove this result in App. \ref{sec:proof-upper-bound}. This theorem highlights the importance of reporting multiple ratings for each preference datapoint, because it shows that when $\alpha(x, y_w, y_l) = 1$, the objectives only have an optimum at infinity.
    %. Most publicly available training datasets have a single rater for each datapoint or only report aggregated preferences, in which case $\alpha(x, y_w, y_l) = 1$ and the RLHF and DPO objectives would only have an optimum at infinity.
\end{remark}

%\sm{Is it possible for us to turn this into an actual upper bound? Could still be that a suboptimal DPO loss value yields a higher ranking acc...}



% \ac{Perhaps this remark below can be moved to the proof in the Appendix? Or a footnote?}
% \begin{remark}
% We note that our result can be straightforwardly derived from many prior fundamental~\citep{peters2007reinforcement} and recent RLHF theory~\citep{korbak2022rl,rafailov2023direct,go2023aligning} works.
% %have derived the optimal target distribution $\pi^\star$. 
% Specifically, when performing RLHF with a reward model (see~\Cref{subsec:prelims_preferences}), the optimal target distribution satisfies $\pi^\star (y |x) = \pi_{ref} (y |x)\exp(r(x, y)/\beta)$, where $r(x, y)$ is the learned reward function. 
% When the reward function obeys the Bradley-Terry model (\Cref{assume:bt}), our result follows straightforwardly from the equivalence of the minimizers of RLHF and DPO.
% % There are some other papers starting from foundamental RL papers \cite{peters2007reinforcement} to recent RLHF theory \cite{korbak2022rl, rafailov2023direct, go2023aligning} that have derived the ideal target distribution. Specifically, when performing RLHF with a reward model, the target distribution satisfies $$\pi^\star \sim \pi_{ref} \exp(r(x)/\beta)$$, where $r(x)$ is the learned reward function. 
% % When the reward model is a Bradley-Terry model, we know that 
% % $$\mathbb{P}(y_w\succ y_l) = \frac{\exp(r(y_w))}{\exp(r(y_w)) \exp(r(y_l))}$$
% % and we can re-derive our previous theorem, using the equivalence of RLHF and DPO \cite{rafailov2023direct}.
% \end{remark}

This result allows us to simulate the policy resulting from perfect optimization of either the RLHF or the DPO learning objective. 
As such, given a reference model $\refmodel$ and preference dataset $\gD$, we can easily measure the \emph{idealized ranking accuracy} of a model.
We prove this result in App.~\ref{sec:proof-cor}.

% TODO: include version for with ties as well
\begin{corollary}[Idealized Ranking Accuracy]\label{cor:idealized_rank_acc}
    Given a reference model $\refmodel$, the DPO or RLHF hyperparameter $\beta$, a dataset of aggregated preferences $\gD=\{(x, y_w, y_l)\}$ and their corresponding rater proportions $\alpha(x, y_w, y_l)$, the ranking accuracy of the optimum of the RLHF or DPO objective $\pi^*$ is given by
    \begin{equation}\label{eq:upper-bound}
        \idealrankacc(\gD;\refmodel) =\underset{(x,y_w,y_l)\sim\gD}{\mathbb{E}} \left[\mathbbm{1}\left[\frac{\refmodel({y_w\mid x})}{\refmodel(y_l\mid x)} \left(\frac{\alpha(x, y_w, y_l)}{1-\alpha(x, y_w, y_l)}\right)^{1/\beta} > 1\right]\right]
    \end{equation}
where $\mathbbm{1}[\cdot]$ is the indicator function. 
%We refer to this ranking accuracy as the \textbf{idealized ranking accuracy}. 
When computed on length-normalized likelihoods from $\tilde\refmodel$, we denote the idealized ranking accuracy as $\tilde\idealrankacc$. 
%\xc{here we might want to state $\alpha$ as given by the dataset}
\end{corollary}


% \xc{Rephrased theorem below}
% \begin{theorem} Fix a reference model $\refmodel$ and a preference datapoint $(x, y_w, y_l)\sim\gD$. Suppose we have a dataset with the following data generating process: the example $(x, y_1, y_2)$ (where $y_1$ is preferred to $y_2$) is generated with probability $\alpha(x, y_1, y_2)$, and $(x, y_2, y_1)$ is generated with probability $1-\alpha(x, y_1, y_2)$. Let $\hat{\alpha}(x, y_1, y_2)$ denote the proportion of raters who prefer $y_1$ in the dataset.  We furthermore assume that each response has at least one rater who labels it as the preferred response in the dataset. Let $\pi^*$ be the model resulting from perfectly minimizing the DPO objective or perfectly maximizing the PPO rewards on the dataset as described in~\Cref{subsec:prelims_preferences}\xc{Comment about expressivity}. Then, letting $y_w$ be the response preferred by more raters, the optimal policy $\pi^*$ satisfies
%     \begin{equation}
%         \frac{\pi^*(y_w\mid x)}{\pi^*(y_l\mid x)} = \frac{\refmodel({y_w\mid x})}{\refmodel(y_l\mid x)} \left(\frac{\hat{\alpha}(x, y_w, y_l)}{1-\hat{\alpha}(x, y_w, y_l)}\right)^{1/\beta}.
%     \end{equation}
%     If there is sufficient data such that with probability at least $1-\delta$, $|\hat{\alpha}(x, y_w, y_l) - \alpha(x, y_w, y_l)| \le \eps$, then 
%         \begin{equation}
%        \frac{\refmodel({y_w\mid x})}{\refmodel(y_l\mid x)} \left(\frac{\alpha(x, y_w, y_l) - \eps}{1-\alpha(x, y_w, y_l)+\eps} \right)^{1/\beta} \le  \frac{\pi^*(y_w\mid x)}{\pi^*(y_l\mid x)} \le \frac{\refmodel({y_w\mid x})}{\refmodel(y_l\mid x)} \left(\frac{\alpha(x, y_w, y_l) + \eps}{1-\alpha(x, y_w, y_l) - \eps}\right)^{1/\beta}.
%     \end{equation}\xc{We can make the $\eps$ here something like $O(n^{-1/4})$ or any $o(n^{-1/2})$}
% \end{theorem}





% We use \Cref{thm:upper_bound} to compute the idealized ranking accuracy that various preference-tuned models could achieve on \sm{alpaca-eval?}
% Differences between theorem and computation:
% \begin{enumerate}
%     \item Needs access to $\alpha$ which is not available for most datasets
%     \item The computation depends on the specific choice of $\beta$ used during RLHF. This is frequently unknown for proprietary models, so we measure the idealized accuracies for a range of $\beta$ values and report the minimum, median, and maximum achievable accuracies.
%     \item Description of how ties are handled
%     \item Again the point about length normalization
%     \item Handling the case of $\alpha=1$
% \end{enumerate}

\subsection{Measuring the Alignment Gap}
Given access to $\pi_\text{Ref}$, $\beta$, and the $\alpha(x,y_w,y_l)$ values for each triple $(x,y_w,y_l)$ in a given preference dataset, we can compute the idealized ranking accuracy from Eq. \ref{eq:upper-bound}.\footnote{Note that when $\alpha(x, y_w, y_l) = 1$, we replace it with $1-\epsilon$ to compute the formula. See App. \ref{app:comp-idealized-ra}.} The results are shown in Table \ref{tab:ranking_accs} and further details are given in App. \ref{app:comp-idealized-ra}.

We identify several surprising findings.
Firstly, even under ideal conditions (\emph{i.e.} perfectly optimizing the objective on ground-truth preference data), the idealized ranking accuracy is still sometimes below $100\%$. 
This distance varies with the choice of $\beta$, which indicates that the limits of DPO/RLHF depend largely upon how strong the reliance on $\pi_\text{Ref}$ is. 
Furthermore, we find that many state-of-the-art models do not achieve a ranking accuracy anywhere close to the idealized ranking accuracy, exhibiting alignment gaps ranging from 19 to 59 percentage points (measured to the median idealized $\rankacc$ or $\tilde\rankacc$).

\fi

==> sections_theoretical_foundations/preliminaries.tex <==
We defer preliminaries on preference learning (data, methods, and evaluations) to App.~\ref{sec:app_preliminaries}.
The current paper primarily studies the DPO objective, though some of our findings extend to RLHF, as noted.
\begin{definition}[DPO Objective~\citep{rafailov2023direct}]\label{def:dpo}
    Let $\sigma$ be the sigmoid function and $\beta>0$ be a hyperparameter. Then, the DPO objective for an aggregated preference dataset $\gD$ (\Cref{def:datapoint}) and a reference model $\refmodel$ is defined as
    \begin{align*}
        &\dpoloss(\model, \refmodel) = \\
        &- \mathbb{E}_{\gD}[\log\sigma(\beta\log\frac{\model(y_w\mid x)}{\refmodel(y_w\mid x)} - \beta\log\frac{\model(y_l\mid x)}{\refmodel(y_l\mid x)})] \\
        % &=- \mathop{\mathbb{E}}_{(x, y_w, y_l)\sim\gD} [\log\sigma(\beta\underbrace{\log\frac{\model(y_w\mid x)}{\model(y_l\mid x)}}_{\text{model log-ratio}} + \beta\underbrace{\log\frac{\refmodel(y_l\mid x)}{\refmodel(y_w\mid x)}}_{\text{reference model log-ratio}})]
    \end{align*}
    We denote the DPO loss on the aggregated datapoint $(x, y_w, y_l)$ as $\dpoloss(x, y_w, y_l; \model, \refmodel)$. 
\end{definition}
As aforementioned, a key metric of the aligned model is the ranking accuracy.
\begin{definition}[Ranking Accuracy]\label{def:ranking_accuracy}
    The ranking accuracy $\rankacc$ of a model $\model$ on an aggregated preference datapoint $(x, y_w, y_l)$ is defined as 
    \begin{equation}
        \rankacc(x, y_w, y_l;\pi_\theta) = \begin{cases} 1 & \model(y_w\mid x) \geq \model(y_l\mid x) \\
        0 & \text{otherwise.} \end{cases}
    \end{equation}
    Analogously, the ranking accuracy of policy $\pi_\theta$ on a dataset $\mathcal{D}=\{(x,y_w,y_l)\}$ is
    $
        \rankacc(\mathcal{D};\pi_\theta)=\E_{(x,y_w,y_l)\sim\mathcal{D}} \rankacc(x,y_w,y_l;\pi_\theta).
    $
    In the rare case where a dataset has more than two outputs $y$ per prompt $x$, we use the generalized ranking accuracy definition stated in App. \ref{app:ra-def-n-greater-than-2}. For completeness, we report the ranking accuracies of both the unnormalized and normalized policies, denoted $\rankacc$ and $\tilde\rankacc$, respectively.
\end{definition}
We initiate an understanding of ranking accuracy by showing that, under the very stringent condition that the reference model already has the correct ranking, minimizing the DPO loss ensures high ranking accuracy.

\begin{proposition}[Sanity Check] Recall the definition of $y_w$, $y_l$ in Definition \ref{def:datapoint}.
    If $\refmodel(y_w\mid x) \geq \refmodel(y_l\mid x)$ and $\dpoloss(x, y_w, y_l; \model, \refmodel) \leq 0.6$, then $\rankacc(x, y_w, y_l) =1$.%\footnote{Proof in \ref{sec:proof-sanity-check}.}
    \label{prop:sanity_check} 
\end{proposition}

==> sections_theoretical_foundations/understanding_ranking_acc.tex <==
%\ac{Add a sentence here explaining that although we analyzed both RLHF and DPO models above, we will focus the rest of our analysis on DPO and here's why.} 
% We now turn to the training objectives to account for the alignment gap.
% %between the idealized setting and real-world results (\Cref{tab:ranking_accs}). 
% We focus our analysis on the DPO objective (\Cref{def:dpo}), because its failure to achieve high ranking accuracy is especially surprising (\Cref{tab:ranking_accs}).
% In particular, DPO directly maximizes the reward margin between preferred-dispreferred  pairs over an offline dataset so we would expect it to perform well on in-distribution held-out data.
% %For example, \Cref{prop:sanity_check} demonstrates that minimizing the loss should correspond to increasing the ranking accuracy.
% %However, \Cref{tab:ranking_accs} demonstrates that models tuned with DPO rarely achieve a high ranking accuracy.
% We also note that DPO is a popular choice in the community for aligning LLMs, because it is less costly than performing RLHF.
\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/log_sft_ratio_vs_loss_3models_seed0.pdf}
    \caption{
    % \textbf{Loss does not correlate with ranking accuracy, but the reference model log-ratio does.}
    % \textbf{Ranking accuracy of the final DPO-trained model is highly dependent on the reference model log-ratio.}
    \textbf{DPO loss alone does not predict ranking accuracy, due to the influence of the reference model log-ratio in the loss.}
    Each point represents the DPO loss on a separate training example $(x,y_w,y_l)$ from a subsample of 1K examples from the training dataset, using the model $\pi_{\theta^*}$ that corresponds to the checkpoint with the lowest validation loss. The color of each point indicates whether $\pi_{\theta^*}$ achieves the correct ranking on that example, \emph{i.e.}, whether $\pi_{\theta^*}(y_w|x)>\pi_{\theta^*}(y_l|x)$. The dashed line is the function $f(c)=-\log\sigma(\beta c)$, from \Cref{prop:dpo_loss}. In summary, the examples that $\pi_{\theta^*}$ classifies correctly tend to be those that were already classified correctly by the reference model. Additional results are in Fig. \ref{fig:dpo-vs-lsr-vs-flipped-other-seeds}.}
    \label{fig:dpo-vs-lsr-vs-flipped}
\end{figure*}

In this section, we study real-world characteristics of DPO.
First, we show empirically that when training GPT-2 \citep{radford2019language}, Pythia 2.8B \citep{biderman2023pythia}, and Llama 2-7B \citep{touvron2023llama} on the Anthropic HH-RLHF \citep{bai2022training} preference dataset, DPO rarely flips the ranking of the two continuations (Fig.~\ref{fig:flipped-vs-not-flipped}, App. \ref{app:dpo-training-details}, and App. \ref{app:dpo-training-dynamics-results}).
Aside from the group of points for which the model unlearns the correct preference ranking, we observe that the loss decreases and the reward margin increases consistently while training, but at the checkpoint with lowest validation loss, less than half of the incorrectly ranked points have been corrected.
This result combined with the observation that reference models exhibit poor ranking accuracy (Sec.~\ref{sec:ref_model_ranking}) provides an explanation for the observed poor ranking accuracies in \Cref{tab:ranking_accs}.


We now formally characterize how hard it is for DPO to correct the ranking of each datapoint. % when training with DPO (\Cref{prop:dpo_loss}).
\begin{theorem}\label{prop:dpo_loss} Consider an aggregated preference datapoint $(x, y_w, y_l)$ such that the reference model log-ratio is some constant $c$, i.e.
$
\log \frac{\refmodel(y_l|x)}{\refmodel(y_w|x)}=c.$
Then, $\rankacc(x, y_w, y_l) = 1$ if and only if $\dpoloss(x, y_w, y_l) \le -\log \sigma (\beta c)$, where $\sigma$ is the sigmoid function.%\footnote{Proof in \ref{sec:proof-dpo-loss}.}
\end{theorem} 
We prove this result in App. \ref{sec:proof-dpo-loss} and extend it to identity preference optimization (IPO, \citet{azar2023general}) in App.~\ref{sec:ipo}.
Our result highlights how the reference model conditions the optimization: as the reference model log-ratio (\Cref{def:dpo}) grows larger, one has to reduce the DPO loss to a dramatically small value to flip the incorrect ranking.
Fig. \ref{fig:dpo-vs-lsr-vs-flipped} visualizes the reference model log-ratio and highlights that datapoints with even mild ranking errors in the reference model will require the loss to be reduced to a very low value in order to flip the ranking. 

% While both RLHF and DPO target the same optimal distribution, their objectives result in different optimization paths; for instance, the PPO objective (\Cref{subsec:prelims_preferences}) involves maximizing reward subject to a divergence constraint with the reference model, whereas the DPO objective (\Cref{def:dpo}) directly maximizes the reward margin between preferred-dispreferred output pairs over an offline dataset. 
% However, even though the DPO objective is designed to optimize the reward margin of a dataset, we find that the resulting model still achieves poor ranking accuracy on held-out data from the same distribution.
% This phenomenon is more surprising 
%The PPO objective does not directly seek to improve preferences over the offline dataset, while the DPO objective directly optimizes for this reward margin for a given distribution yet still achieves poor ranking accuracy on held-out data over the same distribution. Given the latter is a more surprising result, we focus our analysis below on DPO.

% \begin{enumerate}
%     \item Demonstrate low ranking accuracy of different models on different datasets (this can also be Fig 1 of the paper and appear in the midst of the intro)
%     \item Pinpoint that ranking rarely ever flips and that it is easier to flip points that the SFT model is almost correct on
%     \item Theory: loss can go down substantially without flipping the point if the SFT model is ill-conditioned (we define a frontier of this conditioning)
% \end{enumerate}




\iffalse
\subsection{DPO Rarely Flips Preference Rankings}


To study how ranking accuracy changes over the course of DPO training, we train three sizes of models (GPT-2 \citep{radford2019language}, Pythia 2.8B \citep{biderman2023pythia}, and Llama 2-7B \citep{touvron2023llama}) across three seeds each on the Anthropic HH-RLHF \citep{bai2022training} preference dataset and study the ranking accuracy on different partitions of the training dataset. We present the results from training one seed of Pythia 2.8B in Fig. \ref{fig:flipped-vs-not-flipped}, and defer training details to App. \ref{app:dpo-training-details} and results on the other two models to App. \ref{app:dpo-training-dynamics-results}. In Fig. \ref{fig:flipped-vs-not-flipped}, we partition a random subsample of 1K examples from the training dataset into four groups based on whether the reference model $\refmodel$ had the correct ranking and whether the current model $\model$ has the correct ranking.
%(\emph{i.e.} whether $\pi_\text{Ref}(y_w|x)>\pi_\text{Ref}(y_l|x)$) as well as whether the current model has the correct ranking (\emph{i.e.} whether $\pi_\theta(y_w|x)>\pi_\theta(y_l|x)$). For example, the ``incorrect->correct" label denotes that DPO training flipped the model's ranking from incorrect to correct on that example.

Surprisingly, Fig. \ref{fig:flipped-vs-not-flipped} demonstrates that DPO rarely flips the ranking of $(y_w,y_l)$ over the course of training despite consistently reducing the loss $\dpoloss$.
Aside from the group of points for which the model unlearns the correct preference ranking, we observe that the loss decreases and the reward margin increases consistently while training.
However, at the point of lowest validation loss, less than half of the incorrectly ranked points have been flipped to have the correct ranking.
This indicates that the DPO objective is ill-formulated to induce a high ranking accuracy in practice.




\subsection{Analysis: How Easy Is It To Flip A Ranking?} %\xc{Analysis?}}
In the result below, we show that the DPO loss can decrease substantially without any improvement on the ranking accuracy of the model. 
Specifically, the DPO loss that the model needs to reach in order to have the correct ranking on an example $(x, y_w, y_l)$ depends on the quality of the reference model, quantified by the reference model log-ratio. 
This dependence is highly ill-conditioned, whereby using a reference model with moderately incorrect likelihoods assigned to each continuation can effectively prevent DPO from learning the correct ranking.
%We characterize the threshold function $f$, which is a function of the reference model's log-ratio, such that having a DPO loss below the threshold guarantees correct ranking of the example.

%\ac{Add intuition here that this lets us see *even before training* which examples will be more difficult to flip the ranking for. Maybe as a subheader?}
%\sm{TODO do we want to flip the ratio or keep it the same? See DPO objective in~\Cref{def:dpo}}
\begin{theorem}\label{prop:dpo_loss} Consider an aggregated preference datapoint $(x, y_w, y_l)$ such that the reference model log-ratio is some constant $c$, i.e.
$
\log \frac{\refmodel(y_l|x)}{\refmodel(y_w|x)}=c.$
Then, $\rankacc(x, y_w, y_l) = 1$ if and only if $\dpoloss(x, y_w, y_l) \le -\log \sigma (\beta c)$, where $\sigma$ is the sigmoid function.%\footnote{Proof in \ref{sec:proof-dpo-loss}.}
\end{theorem} 

\begin{remark}  
    It is straightforward to extend our analysis to popular variants of DPO. For illustration, we prove an analogous result for identity preference optimization (IPO, \citet{azar2023general}) in App.~\ref{sec:ipo}.
\end{remark}
We prove this result in App. \ref{sec:proof-dpo-loss}.
Our theoretical result allows us to formally identify the points that will be hard to flip in their rankings.
Fig. \ref{fig:dpo-vs-lsr-vs-flipped} visualizes the reference model log-ratio for several settings and highlights that datapoints with even mild ranking errors in the reference model will require the loss to be reduced to a very low value in order to flip the ranking. 
%, showing that many points exhibit a high reference model log-ratio, which means the DPO loss must be very close to zero in order to flip the ranking to be correct.
%Moreover, we see that many datapoints exhibit massive model log-ratio
App. \ref{sec:qualitative} contains examples of hard-to-learn, easy-to-learn, and easy-to-flip datapoints.
We observe that the hard-to-learn datapoints are substantially longer than the easy ones, and that the easy datapoints generally contain less ambiguous preference annotations.
More generally, our result motivates the use of stronger $\pi_\text{Ref}$ models and iterative or on-policy variants of DPO~\citep{tang2024generalized,yuan2024selfrewarding,kim2024sdpo,tran2023iterative}.

%Our findings demonstrate how regularization toward the reference model can prevent the model from learning the correct rankings during DPO.
%In the next section, we will discuss how the DPO objective can be modified to prevent this ill-conditioning.

%\ac{Link to Fig. \ref{fig:dpo-vs-lsr-vs-flipped}}

% \sm{Move this to appendix}
% \begin{proposition}(Generalization to IPO) The Identity Preference Optimization (IPO) loss is defined as $\mathcal{L}_\text{IPO}(x, y_w, y_l)=\left(\log\frac{\pi_\theta(y_w|x)}{\pi_\text{Ref}(y_w|x)}-\log\frac{\pi_\theta(y_l|x)}{\pi_\text{Ref}(y_l|x)}-\frac{1}{2\tau}\right)^2$. Under this loss, if 
% $$\log \frac{\refmodel(y_w|x)}{\refmodel(y_l|x)} < -\frac{1}{2\tau} ,
% $$
% then zero IPO loss implies that $\rankacc(x, y_w, y_l) = 0$. On the other hand, if  $$\log \frac{\refmodel(y_w|x)}{\refmodel(y_l|x)} = c \ge -\frac{1}{2\tau} ,
% $$
% then $\mathcal{L}_\text{IPO}(x, y_w, y_l) \le \left(c + \frac{1}{2\tau}\right)^2$ guarantees that $\rankacc(x, y_w, y_l) = 1$.
% \end{proposition}

% \sm{Look at optimizer states and then decide if we want to do this below thing instead}
% \begin{proposition}[Rephrased to fit the story] For any $\epsilon > 0$, there exists some $f$ such that if the initial ratio $\frac{\refmodel(y_l|x)}{\refmodel(y_w|x)} \leq f(\epsilon)$, then it is possible to achieve $\dpoloss(x, y_w, y_l), \dpoloss'(x, y_w, y_l) \leq \epsilon$ and $\rankacc(x, y_w, y_l) = -1$ 
% \end{proposition}


%Perhaps we can generalize this theorem, even if we don't generalize the experiments, to the general class of IPO \cite{tang2024generalized}

% \paragraph{Attenuating the model's reliance on $\pi_\text{Ref}$}

% Refer to Fig. \ref{fig:gamma-scaling}

\fi

==> sections_theoretical_foundations/win_rate.tex <==
\section{Ranking Accuracy and Win Rate}\label{sec:ra-and-wr}
Our results on ranking accuracy illuminate how well DPO and RLHF can align to preference data, but we have not yet related these insights to how the generative behavior of the model changes during alignment.
%Although we have established a clear relationship between DPO training and ranking accuracy, this does not tell us whether ranking accuracy directly relates to the quality of the model in online settings. 
%In particular, ranking accuracy is a convenient but off-policy metric and is thus not as widely adopted as the on-policy metric of win rate (see Sec.~\ref{sec:eval_metrics}).
%Whereas practitioners typically evaluate preference-tuned models with on-policy metrics (\emph{i.e.} win rate, see ~\Cref{sec:eval_metrics}), ranking accuracy is a convenient but off-policy metric. 
Indeed, one could maximize the ranking accuracy by learning a strong classifier on the preference data, but that model may not generate high-quality text.
Here, we explore the gap between on-policy (i.e., generative) and off-policy (i.e., classification) behaviors of LLMs through the lens of ranking accuracy and win rate.\footnote{Since the DPO objective directly optimizes for ranking accuracy (\cref{prop:sanity_check}), the relationship between these two metrics is a direct reflection of how off-policy training affects on-policy behavior.}
%, adding to the growing body of work discussing the differences between on-policy and off-policy preference learning~\citep{tajwar2024preference,xu2024dpo,tang2024understanding}.
%Recent work has explored the gap between on-policy and off-policy techniques for LLMs~\citep{tajwar2024preference,xu2024dpo,tang2024understanding}, but here, we focus specifically on the previously unexplored relationship between ranking accuracy and win rate. 
%Having established a clear relationship between DPO training and ranking accuracy, we now turn our attention to the commonly used win rate metric (see~\Cref{sec:eval_metrics} for an overview).
%The win rate is the proportion of times one model's generation is preferred to another  (see~\Cref{sec:eval_metrics} for an overview).
%As such, win rate is measured online whereas ranking accuracy is computed offline with respect to the policy (i.e., the language model).
%In this section, we explore how the offline ranking accuracy is related to the online win metric when aligning LLMs.
We study the relationship between win rate and ranking accuracy in two settings: (1) during DPO training, 
%(\cref{sec:wr-vs-ra-during-training}) 
and (2) in a DPO variant modulating the influence of $\pi_\text{Ref}$:
\begin{align*}\label{eq:gamma-scaling}
    &\mathcal{L}_{DPO}^\gamma(\model,\refmodel)= \\
    &- \mathop{\mathbb{E}}_\gD\left[\log\sigma\left(\beta\left(\log\frac{\model(y_w\mid x)}{\model(y_l\mid x)} + \gamma\log\frac{\refmodel(y_l\mid x)}{\refmodel(y_w\mid x)}\right)\right)\right]
\end{align*}
% We measure the win rate on 500 responses to prompts from the training dataset using the Alpaca Eval GPT-4 \citep{li2023alpacaeval} auto-annotator. %Each win rate number is computed from a sample of 500 response pairs.
% %(\cref{sec:attenuating-pi-ref}).
Please see experimental details and figures in App.~\ref{sec:app_win_rate}.

% \paragraph{Setting 1: DPO Training.} 
% We measure the win rate and the ranking accuracy of a Pythia 2.8B model \citep{biderman2023pythia} during DPO training with the same configuration as in \cref{sec:understanding-ra-with-dpo}. See~\cref{fig:ra-wr-during-training} for the results.

% \paragraph{Setting 2: Attenuating the reference model.}
% \Cref{prop:dpo_loss} showed that $\refmodel$ exerts a negative influence on the ranking accuracy in most cases, so we design a new objective that scales the reference model log-ratio in $\dpoloss$ to further characterize how win rate and ranking accuracy relate.
% %In particular, we %apply this scaling 
% %via a constant hyperparameter $\gamma$ and refer to this 
% %modify the objective to be:
% %, where a higher $\gamma$ generally implies a greater influence of the reference policy:
% \begin{equation}\label{eq:gamma-scaling}
%     \mathcal{L}_{DPO}^\gamma(\model,\refmodel)=- \mathop{\mathbb{E}}_{(x, y_w, y_l)\sim\gD}\left[\log\sigma\left(\beta\left(\log\frac{\model(y_w\mid x)}{\model(y_l\mid x)} + \gamma\log\frac{\refmodel(y_l\mid x)}{\refmodel(y_w\mid x)}\right)\right)\right]
% \end{equation}
% Note that $\dpoloss^\gamma = \dpoloss$ (\Cref{def:dpo}) when $\gamma=1$, and a larger value of $\gamma$ increases the role of the reference model.
% Also, $\gamma$ directly scales $c$ in~\Cref{prop:dpo_loss}, thereby controlling how easy it is to fit the data and increase the ranking accuracy.
% We train a range of Pythia-2.8B models using the $\mathcal{L}_{DPO}^\gamma$ objective for $\gamma\in\{0,0.25,0.5,0.75,1.0,1.25,1.5, 1.75, 2.0\}$ and measure the ranking accuracies and win rates of the best model for each $\gamma$ value.\footnote{We use the best hyperparameters obtained from the experiments in Sec. \ref{sec:understanding-ra-with-dpo}.}

\paragraph{Takeaway: Ranking accuracy correlates with win rate when the model is close to the reference model.}
In both settings, we observe that the win rate and ranking accuracy are highly correlated with one another in the early phase of training but become anti-correlated (i.e., ranking accuracy increases but win rate declines) as 
%training continues (\Cref{subfig:ra-and-wr-during-training-train,fig:gamma-scaling}) and 
the model $\model$ moves away from the reference $\refmodel$ (Fig.~\ref{fig:ra-wr-vs-model-dist}).
%, at which point ranking accuracy continues to increase but win rate begins to decline. 
Unlike traditional overfitting, the test loss is continuing to decline at this point (Fig. \ref{subfig:train-and-eval-loss-during-training}).
Experiments in Fig.~\ref{fig:gamma-scaling} with the attenuated objective in \Cref{eq:gamma-scaling} further show that ranking accuracy and win rate trend together when the influence of the reference model is stronger (i.e., $\gamma$ is larger).

%\sm{Need to work on this paragraph}
We speculate that when the model is far from the reference model, regularization toward the reference model can harm the generative capabilities of the model, which are primarily acquired during pre-training.
In other words, the off-policy behavior of the model can no longer predictably describe the on-policy generations when the reference model used in the offline objective is far from the current model.
Our findings confirm the fundamental tradeoff between fitting the preference data and maintaining generative capabilities acquired during pre-training~\citep{jaques2017sequence} and align with prior observations that adding on-policy preference data can make offline learning more effective~\citep{tang2024generalized,yuan2024selfrewarding,kim2024sdpo,tran2023iterative}.

% When $\model$ is far from $\refmodel$, the policy used to generate completions for the win rate metric is very different from the offline dataset used in DPO.
% In that case, the offline training in DPO can no longer predictably affect the generations that win rate is measured on, so the ranking accuracy and the win rate diverge. This is supported by the results of \citet{tang2024generalized}, who find that offline training improves when more on-policy data is added to the training data.



%%%%%%%%%% ANGIE'S VERSION BELOW %%%%%%%%%%%%%%%
\iffalse
%\subsection{Win Rate vs. Ranking Accuracy During DPO Training}\label{sec:wr-vs-ra-during-training}
We measure the win rate and the ranking accuracy of a Pythia 2.8B model \citep{biderman2023pythia} over the course of DPO training with the same configuration as in \cref{sec:understanding-ra-with-dpo}. The results are shown in~\cref{fig:ra-wr-during-training}.
We observe that the win rate and ranking accuracy are highly correlated with one another in the early phase of training but become anti-correlated as training continues (Fig. \ref{subfig:ra-and-wr-during-training-train}) and the model $\model$ moves further away from the reference $\refmodel$ (Fig. \ref{subfig:ra-wr-vs-model-dist-ckpts}). In particular, ranking accuracy continues to increase but win rate begins to decline. This cannot be straightforwardly attributed traditional overfitting, as the test loss is continuing to decline at this point (Fig. \ref{subfig:train-and-eval-loss-during-training}).


When $\model$ is far from $\refmodel$, the policy used to generate completions for the win rate metric is very different from the offline dataset used in DPO.
In that case, the offline training in DPO can no longer predictably affect the generations that win rate is measured on, so the ranking accuracy and the win rate diverge.
%These findings confirm and extend prior works analyzing the difference between online and offline preference learning in LLMs~\citep{tajwar2024preference,xu2024dpo,ahmadian2024basics}.


%\subsection{Win Rate vs. Ranking Accuracy When Modulating the Influence of $\pi_\text{Ref}$}\label{sec:attenuating-pi-ref}

% Since we observed previously that $\pi_\text{Ref}$ exerts a negative influence on the ranking accuracy in most cases, we scale the reference model log-ratio in $\dpoloss$ (\Cref{def:dpo}) to modulate the ranking accuracy and further characterize its relationship with win rate. In particular, we apply this scaling 
% %via a constant hyperparameter $\gamma$ and refer to this 
% in the modified objective as $\mathcal{L}_{DPO}^\gamma$
% %, where a higher $\gamma$ generally implies a greater influence of the reference policy:
% \begin{equation}\label{eq:gamma-scaling}
%     \mathcal{L}_{DPO}^\gamma(\model,\refmodel)=- \mathop{\mathbb{E}}_{(x, y_w, y_l)\sim\gD}\left[\log\sigma\left(\beta\left(\log\frac{\model(y_w\mid x)}{\model(y_l\mid x)} - \gamma\log\frac{\refmodel(y_w\mid x)}{\refmodel(y_l\mid x)}\right)\right)\right]
% \end{equation}
% Note that $\dpoloss^\gamma = \dpoloss$ (\Cref{def:dpo}) when $\gamma=1$, and a larger value of $\gamma$ increases the role of the reference model.
% In other words, $\gamma$ can be seen as directly scaling $c$ in~\Cref{prop:dpo_loss}, thereby controlling how easy it is to learn different datapoints and increase the ranking accuracy.
% We train a range of Pythia-2.8B models using the $\mathcal{L}_{DPO}^\gamma$ objective for $\gamma\in\{0,0.25,0.5,0.75,1.0,1.25,1.5, 1.75, 2.0\}$ and measure the ranking accuracies and win rates of the best model for each $\gamma$ value. 
The results are shown in Fig. \ref{fig:gamma-scaling}. Similar to the previous setting (Sec. \ref{sec:wr-vs-ra-during-training}), ranking accuracy and win rate trend in similar directions for settings where the influence of $\pi_\text{Ref}$ is stronger (\emph{i.e.} higher $\gamma$ values). This is also apparent when we plot both metrics against the distance that the model weights have travelled from $\theta_\text{Ref}$ (the weights of $\pi_\text{Ref}$). Fig. \ref{fig:ra-wr-vs-model-dist} demonstrates that -- in either setting -- ranking accuracy and win rate increase together when $\|\theta-\theta_\text{Ref}\|_2^2$ is small. Past a certain distance, off-policy behavior can no longer predict on-policy performance. 
\fi
